Federated Online and Bandit Convex Optimization

We study the problems of distributed online and bandit convex optimization against an adaptive adversary. We aim to minimize the average regret on $M$ machines working in parallel over $T$ rounds with $R$ intermittent communications. Assuming the underlying cost functions are convex and can be generated adaptively, our results show that collaboration is not beneficial when the machines have access to the first-order gradient information at the queried points. This is in contrast to the case for stochastic functions, where each machine samples the cost functions from a fixed distribution. Furthermore, we delve into the more challenging setting of federated online optimization with bandit (zeroth-order) feedback, where the machines can only access values of the cost functions at the queried points. The key finding here is identifying the high-dimensional regime where collaboration is beneficial and may even lead to a linear speedup in the number of machines. We further illustrate our findings through federated adversarial linear bandits by developing novel distributed single and two-point feedback algorithms. Our work is the first attempt towards a systematic understanding of federated online optimization with limited feedback, and it attains tight regret bounds in the intermittent communication setting for both first and zeroth-order feedback. Our results thus bridge the gap between stochastic and adaptive settings in federated online optimization.

==> related.tex <==
\begin{figure}[!tbh]
    \centering
    \includegraphics[width=0.7\textwidth]{ICML 2023/hierarchy.png}
    \caption{Summary of the problem space of federated online optimization. An arrow from the parent to child denotes that the child min-max problem is easier or has a lower min-max value than the parent problem. Note that to show that there is no benefit of collaboration for first-order algorithms for the problem (P2), we use the lower bound construction for the problem (P5). The figure clarifies why this does not contradict the benefit of collaboration for problems (P9) and (P10), as they lie on a different path from the parent (P2).}
    \label{fig:hierarchy}
\end{figure}
First, we recall that the algorithms on each machine can depend on all the history it has seen. Since we are in the IC setting, at time $t$ on machine $m$, the algorithm $A$'s output can only depend on $$\left(f_1^{1:M}, \ldots, f_{\tau(t)}^{1:M}, f_{\tau(t)+1}^{m},\ldots, f_{t-1}^{m}\right),$$ where $\tau(t)$ is the last time step smaller than or equal to $t$ where communication happened. We also assume that the algorithms can be randomized, i.e., at each time $t$ on machine $m$, the output can also depend on a randomly drawn seed $z_t^m$. With that said, the hardest adversarial problem we can hope to solve for functions coming from some problem class $\ppp\subset \fff^{\otimes MT}$ is
\begin{align}
    \min_{A\in\aaa} \ee_{A}\sb{\max_{P\in \ppp}  \frac{1}{MT}\sum_{t\in [T], m\in[M]}f_t^m(x_t^m) - \min_{x^\star\in \bb_2(B)}\frac{1}{MT}\sum_{t\in [T], m\in[M]}f_t^m(x^\star)}.\tag{\textbf{P1}}
\end{align}

For this problem, note that the max-player knows both the algorithm and the randomization of the min-player. Thus, the min-player doesn't gain from randomization at all. A simpler problem is the following, where the max-player knows the algorithm but not the random seeds
\begin{align}
    \min_{A\in\aaa}\max_{P\in \ppp}  \ee_{A}\sb{\frac{1}{MT}\sum_{t\in [T], m\in[M]}f_t^m(x_t^m) - \min_{x^\star\in \bb_2(B)}\frac{1}{MT}\sum_{t\in [T], m\in[M]}f_t^m(x^\star)}. \tag{\textbf{P2}}
\end{align}
Problem (P2) is usually considered when talking about randomized optimization algorithms. Note that randomization on the second player doesn't increase the min-max regret, so we can equivalently state (P2) with randomized max-players as follows
\begin{align}
    \min_{A\in\aaa}\max_{P\in \ppp}  \ee_{A, P}\sb{\frac{1}{MT}\sum_{t\in [T], m\in[M]}f_t^m(x_t^m) - \min_{x^\star\in \bb_2(B)}\frac{1}{MT}\sum_{t\in [T], m\in[M]}f_t^m(x^\star)}.\tag{\textbf{P2}}
\end{align}
However, making the randomization on the max-player explicit makes it easier to state the following easier version of the problem (P2) with a weaker comparator
\begin{align}
    \min_{A\in\aaa}\max_{P\in \ppp}  \ee_{A}\rb{\ee_P\sb{\frac{1}{MT}\sum_{t\in [T], m\in[M]}f_t^m(x_t^m)} - \min_{x^\star\in \bb_2(B)}\ee_P\sb{\frac{1}{MT}\sum_{t\in [T], m\in[M]}f_t^m(x^\star)}}. \tag{\textbf{P3}}
\end{align}
The comparator in problem (P3) does not know the randomization of the max-player. This form of regret is common in multi-armed bandit literature and is often called \textit{``pseudo-regret"}. In this paper, we upper bound (P2), thus also upper bounding (P3), which might be more relevant for the federated adversarial linear bandits problem. We have only discussed the \textit{``adaptive"} setting so far. We can also relax the problem (P2) by weakening the adversary. One way to do this is by requiring the functions to be the same across the machines, which leads to the following problem
\begin{align*}
    \min_{A\in\aaa}\max_{\{f_t\in\fff\}^{\otimes M}_{t\in[T]}\in \ppp}  \ee_{A}\sb{\frac{1}{MT}\sum_{t\in [T], m\in[M]}f_t(x_t^m) - \min_{x^\star\in \bb_2(B)}\frac{1}{T}\sum_{t\in [T]}f_t(x^\star)}.\tag{\textbf{P4}}
\end{align*}
Note that if the functions across the machines are shared, then $\zeta=0$ in Assumption \ref{ass:heterogeneity}. Depending on the algorithm class, this problem may or may not be equivalent to a fully serial problem, as we showed in this paper. We can further simplify this problem by making the adversary stochastic
\begin{align*}
    \min_{A\in\aaa}\max_{\ddd\in \Delta(\fff)}  \ee_{A, \{f_t\sim \ddd\}_{t\in[T]}}\sb{\frac{1}{MT}\sum_{t\in [T], m\in[M]}f_t(x_t^m) - \min_{x^\star\in \bb_2(B)}\frac{1}{T}\sum_{t\in [T]}f_t(x^\star)}. \tag{\textbf{P5}}
\end{align*}
We can also simplify problem (P5) to have a weaker comparator or consider problem (P3) with a stochastic adversary
\begin{align*}
    \min_{A\in\aaa}\max_{\ddd\in \Delta(\fff)}  \ee_{A, \{f_t\sim \ddd\}_{t\in[T]}}\sb{\frac{1}{MT}\sum_{t\in [T], m\in[M]}\ee_{f_t\sim \ddd}\sb{f_t(x_t^m)}}- \min_{x^\star\in \bb_2(B)}\ee_{f\sim \ddd}\sb{f(x^\star)}. \tag{\textbf{P6}}
\end{align*}
Recalling the definition of $F_m, F$ this can be re-written as,
\begin{align*}
    \min_{A\in\aaa}\max_{\ddd\in \Delta(\fff)}  \ee_{A, \{f_t\sim \ddd\}_{t\in[T]}}\sb{\frac{1}{MT}\sum_{t\in [T], m\in[M]}F(x_t^m)}- \min_{x^\star\in \bb_2(B)}F(x^\star). \tag{\textbf{P6}}
\end{align*}
Now let's relax (P2) directly to have stochastic adversaries, i.e., have fixed distributions on each machine. Note that this will require appropriately changing the problem classes' assumptions, as discussed in the remarks \ref{rem:heterogeneity} and \ref{rem:loss_optimal}.  To simplify the discussion, we assume that the problem class has no additional assumption and is just a selection of $MKR$ functions from some class $\fff$. With this simplification, we can now relax $(P2)$ by picking the functions at machine $m$ at time $t$ from the distribution $\ddd_m$. This leads to the following problem
\begin{align}
    \min_{A\in\aaa}\max_{\{\ddd_m\sim \Delta(\fff)\}_{m\in [M]}}  \ee_{A, \{f_t^m\sim \ddd_m\}_{t\in[T]}^{m\in [M]}}\sb{\frac{1}{MT}\sum_{t\in [T], m\in[M]}f_t^m(x_t^m) - \min_{x^\star\in \bb_2(B)}\frac{1}{MT}\sum_{t\in [T], m\in[M]}f_t^m(x^\star)}. \tag{\textbf{P7}}
\end{align}
If we weaken the comparator for this problem and recall the definitions for $\{F_m := \ee_{f\sim \ddd_m}[f]\}_{m\in[M]}$ and $F := \frac{1}{M}\sum_{m\in[M]}F_m$, we get the following problem
\begin{align}
    \min_{A\in\aaa}\max_{\{\ddd_m\sim \Delta(\fff)\}_{m\in [M]}}  \ee_{A, \{f_t^m\sim \ddd_m\}_{t\in[T]}^{m\in [M]}}\sb{\frac{1}{MT}\sum_{t\in [T], m\in[M]}F_m(x_t^m)} - \min_{x^\star\in \bb_2(B)}F(x^\star). \tag{\textbf{P8}}
\end{align}
We note that problem (P8) is the regret minimization version of the usual heterogeneous federated optimization problem \citep{mcmahan2016communication, woodworth2020minibatch}. To make the final connection to the usual federated optimization literature, we note that the problem becomes easier if the algorithm can look at all the functions before deciding which model to choose. In other words, minimizing regret in the online setting is harder than creating one final retrospective model. This means we can simplify the problem (P8) to the following problem, where $A$ outputs $\hat{x}$ after looking at all the functions
\begin{align}
    \min_{A\in\aaa}\max_{\{\ddd_m\sim \Delta(\fff)\}_{m\in [M]}}  \ee_{A, \{f_t^m\sim \ddd_m\}_{t\in[T]}^{m\in [M]}}\sb{\frac{1}{MT}\sum_{t\in [T], m\in[M]}F_m(\hat{x})} - \min_{x^\star\in \bb_2(B)}F(x^\star). \tag{\textbf{P9}}
\end{align}
With some re-writing of the notation, this reduces the usual heterogeneous federated optimization problem \citep{mcmahan2016communication, woodworth2020minibatch}
\begin{align}
    \min_{A\in\aaa}\max_{\{\ddd_m\sim \Delta(\fff)\}_{m\in [M]}}  \ee_{A, \{f_t^m\sim \ddd_m\}_{t\in[T]}^{m\in [M]}}\sb{F(\hat{x})} - \min_{x^\star\in \bb_2(B)}F(x^\star). \tag{\textbf{P9}}
\end{align}
Assuming $\ddd_m= \ddd$ for all $m\in[M]$ this reduces to the usual homogeneous federated optimization problem \citep{woodworth2020local}
\begin{align*}
    \min_{A\in\aaa}\max_{\ddd\in \Delta(\fff)}  \ee_{A, \{f_t^m\sim \ddd\}^{m\in[M]}_{t\in[T]}}\sb{F(\hat{x})}- \min_{x^\star\in \bb_2(B)}F(x^\star). \tag{\textbf{P10}}
\end{align*}
Note that we can get a similar relaxation of the problem (P6) by converting regret minimization to find a final good solution. The problem will look as follows
\begin{align*}
    \min_{A\in\aaa}\max_{\ddd\in \Delta(\fff)}  \ee_{A, \{f_t\sim \ddd\}_{t\in[T]}}\sb{F(\hat{x})}- \min_{x^\star\in \bb_2(B)}F(x^\star). \tag{\textbf{P11}}
\end{align*}
The key difference between (P10) and (P11) is that $\hat{x}$ depends on $MT$ v/s $T$ samples respectively each case. This means (P10) is simpler than (P11). This concludes the discussion, and we summarize the comparisons between different min-max problems in Figure \ref{fig:hierarchy}. Next, we discuss two relevant lower bounds that follow from this understanding of problem hierarchies. 

\section{Relevant Lower Bound Proofs}\label{sec:lower_bounds}

We would like to understand the lower bounds for the problem (P2) from the previous section, i.e., this paper's main quantity of interest for relevant problem and algorithm classes. Note that to lower bound (P2), we can lower bound any children problems in Figure \ref{fig:hierarchy}. We first restate a well-known OCO sample complexity lower bound to show that 
\begin{align}
  \rrr^1(\ppp_{M,K,R}(\fff^{G, B}, \zeta)) \cong \rrr^1(\ppp_{M,K,R}(\fff^{G, B}_{lin}, \zeta)) \cong \frac{GB}{\sqrt{KR}}. \label{eq:order_independent_lb_lip}
\end{align}

To see this, we recall that $(P2)\succeq (P4) \succeq (P5)$ and then note that for the adversary in $(P5)$, $\zeta=0$ by design as all the machines see the same function. Thus to prove a lower bound, it is sufficient to specify a distribution $\ddd\in \Delta(\fff^{G,B}_{lin})\subset \Delta(\fff^{G,B})$ such that for \textbf{any} sequence of models $\{x_t^m\}_{t\in[T]}^{m\in[M]}$, 
$$\ee_{\{f_t\}_{t\in[T]}}\sb{\frac{1}{MT}\sum_{m,t}f_t(x_t^m) - \min_{x^\star\in \bb_2(B)}\frac{1}{T}\sum_{t}f_t(x^\star)}\succeq \frac{GB}{\sqrt{T}}.$$
And one such easy construction is choosing $f_t(x) = \inner{v_t}{x}$ where $v_t\sim \frac{G}{\sqrt{d}}\cdot Unif(\{+1, -1\}^d)$. This ensures that the first term on the L.H.S. in the above inequality is zero after taking the expectation no matter which model is picked. The minimizer of the second quantity is $x^\star$ is $-\frac{GB}{\sqrt{T}}$ (c.f., Theorem 3.2 \citep{hazan2016introduction}), which gives the lower bound in equation \eqref{eq:order_independent_lb_lip}. Note that the construction is linear and lies in the class $\fff^{G,B}$, which is an order-optimal lower bound since it doesn't have anything to do with the form of the algorithm. Furthermore, to get equality in equation \eqref{eq:order_independent_lb_lip}, we recall the non-collaborative OGD upper bound (c.f., Theorem 3.1 \citep{hazan2016introduction}). 

Next, we draw our attention to the problem class of smooth functions $\ppp_{M,K,R}(\fff^{H,B}, \zeta, F_\star)$ where we show that 
\begin{align}
\rrr^1(\ppp_{M,K,R}(\fff^{H,B}, \zeta, F_\star)) \cong \frac{HB^2}{T} + \frac{\sqrt{HF_\star}B}{\sqrt{T}}. \label{eq:order_independent_lb_smth}
\end{align}
We use the same lower-bounding strategy mentioned above but instead lower bound (P10), and note that $(P2)\succeq (P4) \succeq (P5) \succeq (P6) \succeq (P10)$. This already makes $\zeta=0$ since our attack is coordinated. To lower bound (P10), we use the construction and distribution as used in the proof of Theorem 4 by \citet{woodworth2021even}, which is a sample complexity lower bound that only depends on $T$, i.e., the number of samples observed from $\ddd$. For the upper bound, we use Theorem 3 by \citet{srebro2010optimistic} proved in the same setting. Even though the upper bounds are first-order algorithms, the lower bounds are order-independent, i.e., sample complexity lower bounds. 

Finally, we'd like to prove a lower bound for the problem class $\ppp_{MKR}(\fff^{G,B})$ with two-point bandit feedback. In particular, we want to show that
\begin{align}
\rrr^{0,2}(\ppp_{MKR}(\fff^{G,B}), \zeta) \succeq \frac{GB}{\sqrt{KR}} + \frac{GB\sqrt{d}}{\sqrt{MKR}}.
\end{align}
To prove this, we'd use the reduction $(P2)\succeq (P4) \succeq (P5) \succeq (P6)$. Then we note for the problem (P6), $\zeta=0$, and using $2$-point feedback; we get in total $2MKR$ function value accesses to $\ddd$. We can use the lower bound in Proposition 2 by \citet{duchi2015optimal} for the problem (P6) for $2M$ points of feedback and $KR$ iterations. Combined with the order-independent lower bound proved previously, this proves the required result.  



==> setting.tex <==
 This section introduces definitions and assumptions used in our analysis. We formalize our adversary class and algorithm class. We also specify the notion of min-max regret.% we want to study.

% \red{lets have the notation section here? it looks out of place if we put it at the end of Sec 1. I moved once before, also, is that fine?} 
\paragraph{\textbf{Notation.}} We denote the horizon by $T=KR$.  $\succeq, \preceq, \cong$ denote inequalities up to numerical constants. We denote the average function by $f_t(\cdot)~:=~\sum_{m\in[M]}f_t^m(\cdot)/M$ for all $t\in[T]$. We use $\mathbbm{1}_{A}$ to denote the indicator function for the event $A$. $\bb_2(B)\subset \rr^d$ denotes the $L_2$ ball of radius $B$ centered at zero. We suppress the indexing in the summation $\sum_{t\in[T], m\in[M]}$ to $\sum_{t,m}$ due to space constraints wherever the usage is clear.


\paragraph{\textbf{Function Classes.}} We consider several common function classes \citep{saha2011improved, hazan2016introduction} in this paper:
\begin{enumerate}
    \item $\boldsymbol{\fff^{G, B}}$, the class of convex, differentiable, and $G$-Lipschitz functions, i.e., $$\forall x,y\in\rr^d,\ |f(x)-f(y)|\leq G\norm{x-y}$$ with bounded optima $x^\star\in \bb_2(B)$.
    \item $\boldsymbol{\fff^{H, B}}$, the class of convex, differentiable, and $H$-smooth functions, i.e., $$\forall x,y\in\rr^d,\ \norm{\nabla f(x)-\nabla f(y)}\leq H\norm{x-y}$$ with bounded optima $x^\star\in \bb_2(B)$. We also define $\boldsymbol{\fff^{G, H, B}} := \boldsymbol{\fff^{G, B}}\cap \boldsymbol{\fff^{H, B}}$, i.e., the class of Lipschitz and smooth functions.
    \item $\boldsymbol{\fff_{lin}^{G, B}} \subset \boldsymbol{\fff^{G, B}}$, which includes linear cost functions with gradients bounded by $G$. This includes the cost functions in federated adversarial linear bandits, discussed in Section \ref{sec:falb}.
    % \lnote{we should be careful about the $x \in \xxx$ in linear case, since the query with random $u$ may outside $\xxx$, and we cannot claim to project to a smaller ball since $x^\star$ is in $\xxx$ instead of the small ball. Should we just define $x^\star$ in $\xxx$ instead of any $x\in \xxx$?}
\end{enumerate}
\todo{Do we need to have the bounded comparator condition in the function class definition?}

% \\ (i) $\boldsymbol{\fff^{G, B}}$, the class of convex, differentiable, and $G$-Lipschitz functions, i.e., $$\forall x,y\in\xxx,\ |f(x)-f(y)|\leq G\norm{x-y},$$ with bounded optima, $x^\star\in \xxx$;\\ 
% (ii) $\boldsymbol{\fff^{H, B}}$, the class of convex, differentiable, non-negative and $H$-smooth functions, i.e., $$\forall x,y\in\xxx,\ \norm{\nabla f(x)-\nabla f(y)}\leq H\norm{x-y}$$ with bounded optima $x^\star\in \xxx$;\\
% (iii) $\boldsymbol{\fff_{lin}^{G, B}} \subset \boldsymbol{\fff^{G, B}}$ which includes linear cost functions with gradients bounded by $G$. We also define $\boldsymbol{\fff^{G, H, B}} := \boldsymbol{\fff^{G, B}}\cap \boldsymbol{\fff^{H, B}}$ and note that $\boldsymbol{\fff_{lin}^{G, B}} \subseteq \boldsymbol{\fff^{G, 0, B}}$.


\paragraph{\textbf{Adversary Model.}} Note that in the most general setting, each machine will encounter arbitrary functions from a class $\fff$ at each time step. Our algorithmic results are for this general model, which is usually referred to as an \textbf{\textit{``adaptive"}} adversary. Specifically, we allow the adversary's functions to depend on the past sequence of models played by the machines but not on the randomness used by the machines, i.e., $\{f^m_t\}^{m\in[M]}$ for all $t$ can depend on $\big(\{x_i^m\}_{i\in[t-1]}^{m\in[M]}, A\big)$, where $A$ is the algorithm being used by the machines. 

We also consider a weaker \textbf{\textit{``stochastic"}} adversary model to explain some baseline results. More specifically, the adversary cannot adapt to the sequence of the models used by each machine but must fix a distribution in advance for each machine, i.e., $\forall m\in[M],\ \ddd_m\in \Delta(\fff)$ such that at each time $t\in[T]$, $f_t^m\sim \ddd_m$. An example of this less challenging model is \textit{distributed stochastic optimization} where $f_t^m(\cdot):= f(\cdot; z_t^m\sim \ddd_m)$ for $f(\cdot;\cdot)\in \fff$ and $z_t^m$ is a data-point sampled from the distribution $\ddd_m$. For the stochastic adversaries throughout we denote $$F_m(x) := \ee_{f\sim \ddd_m}[f(x)],\ F(x) := \frac{1}{M}\sum_{m\in[M]}F_m(x),$$ where with a slight abuse of notation we suppress $z\sim \ddd_m$. The distinction between different adversary models is discussed further in Appendix \ref{sec:related}.
  

\paragraph{\textbf{Oracle Model.}} We consider three kinds of access to the cost functions in this paper. Each machine $m\in[M]$ for all time steps $t\in[T]$ has access to one of the following:
\begin{enumerate}
\item \textbf{Gradient} of $f_t^m$ at a single point, a.k.a., first-order feedback.
\item \textbf{Function value} of $f_t^m$ at a single point, a.k.a., one-point bandit feedback.
\item \textbf{Function values} of $f_t^m$ at two different points, a.k.a., two-point bandit feedback. 
\end{enumerate}
% \\ (i) \textbf{gradient} of $f_t^m$ at one point, a.k.a., first-order feedback;\\ (ii) \textbf{function value} of $f_t^m$ at one point, a.k.a., bandit feedback;\\ (iii) \textbf{function values} of $f_t^m$ at two different points, a.k.a., two-point bandit feedback. 
\begin{remark}
Note that we always look at the regret at the queried points. Thus in the two-point feedback setting, if the machine $m$ queries at points $x_t^{m,1}$ and $x_t^{m,2}$ at time $t$, it incurs the cost $f_t^m(x_t^{m,1}) + f_t^m(x_t^{m,2})$ (c.f., Theorem \ref{thm:bd_grad_first_stoch}).
\end{remark}
\textbf{Algorithm Class.} We assume the algorithms on each machine can depend on all the history it has seen. Since we are in the IC setting, at time $t$ on machine $m$, the algorithm $A$'s output can only depend on $$\left(f_1^{1:M}, \ldots, f_{\tau(t)}^{1:M}, f_{\tau(t)+1}^{m},\ldots, f_{t-1}^{m}\right),$$ where $\tau(t)$ is the last time step smaller than or equal to $t$ where communication happened. We assume $T=KR$ so that $\tau(t) := t \mod K$. In other words, the algorithms' output on a machine can depend on all the information (gradients or function values) it has seen on the machine or other machines' information communicated to it. We denote this class of algorithms by $\aaa_{IC}$ and add super-scripts $1$, $0$, $(0,2)$ to denote first-order, one-point bandit, and two-point bandit feedback. Thus, we consider three algorithm classes $\aaa_{IC}^1,\ \aaa_{IC}^0,\ \aaa_{IC}^{0,2}$ in this paper.

Finally, we consider two more assumptions controlling how similar the cost functions look across machines and the average regret at the comparator \citep{srebro2010optimistic}:

% \red{AS: I suggest we add a title/small description for each Assumption, Thm, Rem, I did for a few.}

\begin{assumption}[Bounded First-Order Heterogeneity]
\label{ass:heterogeneity}
For all $t\in [T],\ x\in \rr^d$, $$\frac{1}{M}\sum_{m\in[M]}\norm{\nabla f_t^m(x)- \nabla f_t(x)}^2 \leq \zeta^2\leq 4G^2.$$
\end{assumption}

% \red{is this remark needed?}
\begin{remark}[Bounded First-Order Heterogeneity for Stochastic Setting]\label{rem:heterogeneity}
    In the stochastic setting, \citet{woodworth2020minibatch} consider a related but more relaxed assumption, i.e.,  $\forall\ x\in\rr^d$, $$\frac{1}{M}\sum_{m\in[M]}\norm{\nabla F_m(x) - \nabla F(x)}^2 \leq \zeta^2\leq 4G^2.$$ This assumption does not require the gradients at each time step to be point-wise close but requires them to be close only on average over the draws from the machines' distributions.
\end{remark}

% \red{AS: Can we use a separate counter for the Assumptions, eg, Assumption 1 , 2. The current numbering looks confusing. Rem \& Assumption numbering should not be tied together}\lnote{note sure about this since the default icml template use this}

\begin{assumption}[Bounded Optimality at Optima]
\label{ass:loss_optimal}
For all $x^\star\in \arg\min_{x\in \bb_2(B)}\sum_{t\in [T]}f_t(x),$ $$\frac{1}{T}\sum_{t\in[T]}f_t(x^\star)~\leq~F_\star.$$ For non-negative functions in $\fff^{H, B}$, this implies, $$\frac{1}{T}\sum_{t\in[T]}\norm{\nabla f_t(x^\star)}^2~\leq~HF_\star,$$ (c.f., Lemma 4.1 in \citet{srebro2010optimistic}).
\end{assumption}
\todo{Maybe we should define this as an irreducible loss instead of an assumption?}

\begin{remark}[Bounded Optimiality for Stochastic Setting]\label{rem:loss_optimal}
When the functions are generated stochastically, denote $F_\star:= \min_{x\in \bb_2(B)}F(x)$ as the minimum realizable function value. Then assuming $\ddd_m$ is supported on functions in $\fff^{H, B}$, implies for all $t\in[T]$, $$\ee_{\{f_t^m\sim \ddd_m\}_{m\in[M]}}\norm{\frac{1}{M}\sum_{m\in[M]}\nabla f_t^m(x^\star)}^2~\leq~HF_\star$$ (c.f., Lemma 3 in \citet{woodworth2021even}).
\end{remark}


\paragraph{\textbf{Min-Max Regret.}} We now define our problem class. We use $\ppp_{M, K, R}(\fff) := \fff^{\otimes MKR}$ to denote all selections of $MKR$ functions from a class $\fff$. We use the argument $\zeta$, $F_\star$ to further restrict this to selections that satisfy Assumptions \ref{ass:heterogeneity} and \ref{ass:loss_optimal} respectively. In this paper, we consider four problem classes: $$\ppp_{M, K, R}(\fff^{G, B}, \zeta),\ \ppp_{M, K, R}(\fff^{H, B}, \zeta, F_\star),\ \ppp_{M, K, R}(\fff^{G, H, B}, \zeta, F_\star), \text{ and } \ppp_{M, K, R}(\fff^{G, B}_{lin}, \zeta).$$ We are interested in characterizing the min-max regret for these classes. In particular, for a problem class $\ppp$ and algorithm class $\aaa$, we want to characterize up to numerical constants the following quantity:
% \newpage
% \begin{align}\label{eq:P1}
%     \rrr(\ppp) :=
%     &\min_{A\in\aaa} \max_{P\in \ppp} \ee_{A}\Bigg(\frac{1}{MT}\sum_{t\in [T], m\in[M]}f_t^m(x_t^m)\nonumber\\ 
%     &\qquad- \min_{x^\star\in \bb_2(B)}\frac{1}{MT}\sum_{t\in [T], m\in[M]}f_t^m(x^\star)\Bigg),
% \end{align}

\begin{align}\label{eq:P1}
    \rrr(\ppp) := \min_{A\in\aaa} \max_{P\in \ppp} \ee_{A}\frac{1}{MT}\rb{\sum_{t\in [T], m\in[M]}f_t^m(x_t^m)- \min_{x^\star\in \bb_2(B)}\sum_{t\in [T], m\in[M]}f_t^m(x^\star)},
\end{align}
where $A$ is a randomized algorithm producing models $x_t^m$'s. We add super-scripts $0$, $(0,2)$, $1$ to $\rrr$ to denote the algorithm class, i.e.,  $\aaa_{IC}^0,\ \aaa_{IC}^{0,2},\ \aaa_{IC}^1$ respectively. 

The second player, i.e., the adversary selecting the functions, does not benefit from randomization for problem \eqref{eq:P1}, which is why we ignore that here\footnote{It makes sense to make the randomization on the second player explicit when comparing to a weaker comparator, c.f., problem (P3) in Appendix \ref{sec:related}.}. It is also important to note that the max player does not have access to the randomness of the min player (c.f., problem (P1) in appendix \ref{sec:related}). Finally, note again that the max player can adapt to the sequence of models played by $A$, which is why we call this regret minimization against an adaptive adversary. In this paper, we want to characterize the min-max value of this game, i.e., $\rrr(\ppp)$. 

Most existing work \citep{khaled2020tighter,woodworth2020minibatch, patel2022towards, wang2022unreasonable} in federated learning has instead focused on characterizing the min-max regret for the following simpler problem\footnote{These works aim to upper bound the function sub-optimality at a single point, but most of their analyses actually provide regret guarantees that are converted to function sub-optimality bounds at the averaged iterate by applying Jensen's inequality.}:
\begin{align}
    & \rrr_{stoc.}(\ppp)\nonumber := 
    \\
    &\min_{A\in\aaa} \max_{\{\ddd_m\in \Delta(\fff)\}} \ee_{A, \{f_t^m\sim \ddd_m\}_{t\in[T]}^{m\in[M]}} \rb{\frac{1}{MT}\sum_{t, m}f_t^m(x_t^m) - \min_{x^\star\in \bb_2(B)}\frac{1}{MT}\sum_{t, m}\ee_{f_t^m\sim \ddd_m}[f_t^m(x^\star)]}\nonumber\\
    &= \min_{A\in\aaa} \max_{\{\ddd_m\in \Delta(\fff)\}} \ee_{A} \rb{\frac{1}{MT}\sum_{t, m}\ee_{f_{t}^m\sim \ddd_m}[f_t^m(x_t^m)] - \min_{x^\star\in \bb_2(B)}\frac{1}{MT}\sum_{t, m}\ee_{f_t^m\sim \ddd_m}[f_t^m(x^\star)]}\nonumber\\
    &= \min_{A\in\aaa} \max_{\{\ddd_m\in \Delta(\fff)\}}  \ee_{A}\rb{\frac{1}{MT}\sum_{t, m}F_m(x_t^m) - \min_{x^\star\in \bb_2(B)}\frac{1}{M}\sum_{m}F_m(x^\star)},
\end{align}
where $F_m(\cdot) := \ee_{f\sim \ddd_m}[f(\cdot)]$. This problem has a ``stochastic" adversary. The min-max complexity of this easier problem is understood in the ``homogeneous" setting when the machines have the same distribution \citep{woodworth2021min, woodworth2021minimax}. However, it is not yet fully understood in the ``heterogeneous'' setting where these distributions can differ across the machines \citep{woodworth2020minibatch, wang2022unreasonable, glasgow2022sharp}. In general, note that for any problem class $\ppp$, $\rrr_{stoc.}(\ppp)\leq \rrr(\ppp)$, and we are interested in understanding the higher $\rrr(\ppp)$. We further discuss some related distributed problems and their potential applications in Appendix \ref{sec:related}.

% \begin{align}
%     &\rrr_{stoc.}(\ppp):= \nonumber\\ 
%     &\min_{\mathclap{A\in\aaa}} \max_{\mathclap{\ddd_m}} \underset{A}{\ee}\frac{1}{MT} \Bigg(\sum_{t, m}\underset{f_t^m\sim \ddd_m}{\ee}[f_t^m(x_t^m)]\nonumber\\ 
%     &\qquad\qquad\qquad- \min_{x^\star\in \bb_2(B)}\sum_{t, m}\underset{f_t^m\sim \ddd_m}{\ee}[f_t^m(x^\star)]\Bigg)\nonumber\\
%     &= \min_{A\in\aaa} \max_{\{\ddd_m\in \Delta(\fff)\}}  \Bigg(\frac{1}{MT}\sum_{t, m}\ee_{A}[F_m(x_t^m)]\nonumber\\
%     &\qquad\qquad\qquad\qquad - \min_{x^\star\in \bb_2(B)}\frac{1}{M}\sum_{m}F_m(x^\star)\Bigg),
% \end{align}

 
